Dilatation of Lateral Ventricles with Brain Volumes in Infants with 3D Transfontanelle US

Ultrasound (US) can be used to assess brain development in newborns, as MRI is challenging due to immobilization issues, and may require sedation. Dilatation of the lateral ventricles in the brain is a risk factor for poorer neurodevelopment outcomes in infants. Hence, 3D US has the ability to assess the volume of the lateral ventricles similar to clinically standard MRI, but manual segmentation is time consuming. The objective of this study is to develop an approach quantifying the ratio of lateral ventricular dilatation with respect to total brain volume using 3D US, which can assess the severity of macrocephaly. Automatic segmentation of the lateral ventricles is achieved with a multi-atlas deformable registration approach using locally linear correlation metrics for US-MRI fusion, followed by a refinement step using deformable mesh models. Total brain volume is estimated using a 3D ellipsoid modeling approach. Validation was performed on a cohort of 12 infants, ranging from 2 to 8.5 months old, where 3D US and MRI were used to compare brain volumes and segmented lateral ventricles. Automatically extracted volumes from 3D US show a high correlation and no statistically significant difference when compared to ground truth measurements. Differences in volume ratios was 6.0 +/- 4.8% compared to MRI, while lateral ventricular segmentation yielded a mean Dice coefficient of 70.8 +/- 3.6% and a mean absolute distance (MAD) of 0.88 +/- 0.2mm, demonstrating the clinical benefit of this tool in paediatric ultrasound.

==> format.tex <==
\pdfminorversion=5
\usepackage{float}
\usepackage{hyperref}
\usepackage{wrapfig}

\makeatletter%
\hypersetup{%
colorlinks=true,% Colors the text of links and anchors
linkcolor=blue,% Color for normal internal links
citecolor=blue,% Color for bibliographical citations in text
urlcolor=blue,% Color for linked URLs
}%
\makeatother%

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage[usenames,dvipsnames]{color}
\usepackage{ifthen}
\usepackage{array}
\usepackage{wrapfig}
\usepackage{multirow} 
\usepackage{ulem}
\usepackage{subfigure}
\usepackage{verbatim}

%\usepackage{geometry}
%\geometry{hmargin=2.5cm,vmargin=2.4cm}

\usepackage{textcomp} % for symbols
%\usepackage{rotating}


\tolerance=10000000 % related to hyphenation


\hyphenation{liver} 
%\hyphenation{fortran er-go-no-mic} 
% indicates that "fortran" cannot be hyphenated and indicates allowed hyphenation points for "ergonomic"

%
%\makeatletter
%\def\ps@pprintTitle{%
% \let\@oddhead\@empty
% \let\@evenhead\@empty
% \def\@oddfoot{}%
% \let\@evenfoot\@oddfoot}
%\makeatother
%
%\makeatletter
%\renewcommand\section{\@startsection{section}{1}{\z@}{6px}{3px}{\bfseries}}
%\renewcommand\subsection{\@startsection{subsection}{2}{\z@}{0px}{-10px}{\itshape}}
%\makeatother


\newcommand{\margrem}[1]{\normalmarginpar{\marginpar[\parbox{2.0cm}{\raggedleft\tiny{}#1}\tiny~\vrule]{\tiny\vrule~\parbox{3.5cm}{\raggedright\tiny{}#1}}}}
\newcommand{\margecomm}[1]{\protect \margrem{#1}}%

\newcommand{\colorRP}[1]{{\color[rgb]{0.5,0.0,0.5}{#1}}}
\newcommand{\colorSC}[1]{{\color[rgb]{1.0,0.0,1.0}{#1}}}
\newcommand{\colorIP}[1]{{\color[rgb]{0.0,1.0,0.0}{#1}}}
\newcommand{\colorHC}[1]{{\color[rgb]{0.5,0.5,0.0}{#1}}}
\newcommand{\colorRT}[1]{{\color[rgb]{0.5,0.5,0.0}{#1}}}

\newcommand{\RP}[2]{\colorRP{#1}{\margecomm{\colorRP{RP: #2}}}}
\newcommand{\SC}[2]{\colorSC{#1}{\margecomm{\colorSC{SC: #2}}}}
\newcommand{\IP}[2]{\colorIP{#1}{\margecomm{\colorIP{IP: #2}}}}
\newcommand{\HC}[2]{\colorHC{#1}{\margecomm{\colorHC{HC: #2}}}}
\newcommand{\RT}[2]{\colorRT{#1}{\margecomm{\colorRT{RT: #2}}}}

